Learning Deep Multimodal Feature Representation with Asymmetric Multi-layer Fusion

We propose a compact and effective framework to fuse multimodal features at multiple layers in a single network. The framework consists of two innovative fusion schemes. Firstly, unlike existing multimodal methods that necessitate individual encoders for different modalities, we verify that multimodal features can be learnt within a shared single network by merely maintaining modality-specific batch normalization layers in the encoder, which also enables implicit fusion via joint feature representation learning. Secondly, we propose a bidirectional multi-layer fusion scheme, where multimodal features can be exploited progressively. To take advantage of such scheme, we introduce two asymmetric fusion operations including channel shuffle and pixel shift, which learn different fused features with respect to different fusion directions. These two operations are parameter-free and strengthen the multimodal feature interactions across channels as well as enhance the spatial feature discrimination within channels. We conduct extensive experiments on semantic segmentation and image translation tasks, based on three publicly available datasets covering diverse modalities. Results indicate that our proposed framework is general, compact and is superior to state-of-the-art fusion frameworks.

==> tabs/arch.tex <==
\begin{table}[t]
	\begin{center}
		\caption{\textmd{Modified RefineNet with ResNet101 and ResNet152 as backbones respectively. We substitute the last building blocks at the four downsampling stages of ResNet with our fusion blocks, illustrated in Figure 3(c) of our main paper. The input image size in our setting is $500\times500$, and we use this input size as an example to show image sizes at different layers.}}
    	\label{tab-net}
		\resizebox{80mm}{!}{
		\begin{tabular}{c|c|c|c}
			\toprule
			Layer name & ResNet101 & ResNet152 & Output size \\
            \midrule
			$\text{conv}_1$ & \multicolumn{2}{c|}{$7\times 7$, stride 2} & 64$\times$250$\times$250 \\
			\midrule
			$\text{pool}_1$ & \multicolumn{2}{c|}{$3\times 3$ max, stride 2} & 64$\times$125$\times$125 \\
			\midrule
			$\text{res}_2$ & \makecell[c]{standard block $\times$2 \\fusion block $\times$1} & \makecell[c]{standard block $\times$2 \\fusion block $\times$1} & 256$\times$125$\times$125 \\
			\midrule
			$\text{res}_3$ & \makecell[c]{standard block $\times$3 \\fusion block $\times$1} & \makecell[c]{standard block $\times$3 \\fusion block $\times$1}  & 512$\times$63$\times$ 63 \\
			\midrule
			$\text{res}_4$ & \makecell[c]{standard block $\times$22 \\fusion block $\times$1} & \makecell[c]{standard block $\times$35 \\fusion block $\times$1}  & 1024$\times$32$\times$32 \\
			\midrule
			$\text{res}_5$ & \makecell[c]{standard block $\times$2 \\fusion block $\times$1} & \makecell[c]{standard block $\times$2 \\fusion block $\times$1}  & 2048$\times$16$\times$ 16 \\
			\midrule
			\multicolumn{3}{c|}{RefineNet decoder} &40$\times$125$\times$ 125 \\
			\bottomrule
		\end{tabular}}
	\end{center}
\vspace{-2mm}
\end{table}


\iffalse
\begin{table}[t]
	\begin{center}
		\caption{\textmd{Incorporation asymmetric fusion blocks into backbone networks including ResNet101, ResNet152 and Xception65. We substitute the last building blocks at the four downsampling stages of ResNet with our fusion blocks, illustrated in Figure \ref{shuffle_shift}(c).}}
    	\label{tab-net}
		\resizebox{80mm}{!}{
		\begin{tabular}{c|c|c|c}
			\toprule
			Layer name & ResNet101 & ResNet152 & Output size \\
            \midrule
			$\text{conv}_1$ & \multicolumn{2}{c|}{$7\times 7$, stride 2} & 64$\times$8$\times$112$\times$112 \\
			\midrule
			$\text{pool}_1$ & \multicolumn{2}{c|}{$3\times 3$ max, stride 2} & 64$\times$8$\times$56$\times$56 \\
			\midrule
			$\text{res}_2$ & \makecell[c]{standard block $\times$2 \\fusion block $\times$1} & \makecell[c]{standard block $\times$2 \\fusion block $\times$1} & 256$\times$8$\times$56$\times$ 56 \\
			\midrule
			$\text{res}_3$ & \makecell[c]{standard block $\times$3 \\fusion block $\times$1} & \makecell[c]{standard block $\times$3 \\fusion block $\times$1}  & 512$\times$8$\times$28$\times$ 28 \\
			\midrule
			$\text{res}_4$ & \makecell[c]{standard block $\times$22 \\fusion block $\times$1} & \makecell[c]{standard block $\times$35 \\fusion block $\times$1}  & 1024$\times$8$\times$14$\times$ 14 \\
			\midrule
			$\text{res}_5$ & \makecell[c]{standard block $\times$2 \\fusion block $\times$1} & \makecell[c]{standard block $\times$2 \\fusion block $\times$1}  & 2048$\times$8$\times$7$\times$ 7 \\
			\midrule
			\multicolumn{3}{c|}{RefineNet decoder} &- \\
			\bottomrule
		\end{tabular}}
	\end{center}
\vspace{-3mm}
\end{table}
\fi
